Novel utilization of a paper-level classification system for the evaluation of journal impact: An update of the CAS Journal Ranking

Since its first release in 2004, the CAS Journal Ranking, a ranking system of journals based on a citation impact indicator, has been widely used both in selecting journals when submitting manuscripts and conducting research evaluation in China This paper introduces an upgraded version of the CAS Journal Ranking released in 2020 and the corresponding improvements. We will discuss the following improvements: (1) the CWTS paper-level classification system, a fine-grained classification system, utilized for field normalization, (2) the Field Normalized Citation Success Index (FNCSI), an indicator which is robust against not only extremely highly cited publications, but also wrongly assigned document types, and (3) document type difference. In addition, this paper will present part of the ranking results and an interpretation of the features of the FNCSI indicator.

==> CAS Journal Ranking/table/top20.tex <==
\begin{tabular}{|p{4cm}|p{6cm}|p{1.2cm}|p{1.2cm}|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Journal} & \textbf{Category-WoS}                                                                               & \textbf{FNCSI} & \textbf{FNIF} \\ \hline
LANCET               & MEDICINE, GENERAL \& INTERNAL                  & 1  & 3  \\ \hline
NATURE               & MULTIDISCIPLINARY SCIENCES                     & 2  & 5  \\ \hline
JAMA  & MEDICINE, GENERAL \& INTERNAL                  & 3  & 4  \\ \hline
SCIENCE              & MULTIDISCIPLINARY SCIENCES                     & 4  & 9  \\ \hline
CELL                 & BIOCHEMISTRY \& MOLECULAR BIOLOGY/CELL BIOLOGY & 5  & 15 \\ \hline
WORLD PSYCHIATRY     & PSYCHIATRY                                     & 6  & 8  \\ \hline
LANCET NEUROL        & CLINICAL NEUROLOGY                             & 7  & 11 \\ \hline
NAT PHOTONICS        & OPTICS/PHYSICS, APPLIED                        & 8  & 17 \\ \hline
NAT GENET            & GENETICS \& HEREDITY                           & 9  & 13 \\ \hline
NAT MED          & BIOCHEMISTRY \& MOLECULAR BIOLOGY/CELL BIOLOGY/MEDICINE, RESEARCH \& EXPERIMENTAL                   & 10                  & 21                 \\ \hline
NAT MATER        & MATERIALS SCIENCE, MULTIDISCIPLINARY/CHEMISTRY, PHYSICAL/PHYSICS, APPLIED/PHYSICS, CONDENSED MATTER & 11                  & 12                 \\ \hline
LANCET ONCOL         & ONCOLOGY                                       & 12 & 10 \\ \hline
CANCER CELL          & ONCOLOGY/CELL BIOLOGY                          & 13 & 38 \\ \hline
NAT CHEM             & CHEMISTRY, MULTIDISCIPLINARY                   & 14 & 31 \\ \hline
NAT NEUROSCI         & NEUROSCIENCES                                  & 15 & 36 \\ \hline
CELL METAB           & CELL BIOLOGY/ENDOCRINOLOGY \& METABOLISM       & 16 & 51 \\ \hline
LANCET RESP MED  & CRITICAL CARE MEDICINE/RESPIRATORY SYSTEM                                                           & 17                  & 22                 \\ \hline
NAT IMMUNOL          & IMMUNOLOGY                                     & 18 & 58 \\ \hline
LANCET DIABETES ENDO & ENDOCRINOLOGY \& METABOLISM                    & 19 & 27 \\ \hline
NAT NANOTECHNOL  & NANOSCIENCE \& NANOTECHNOLOGY/MATERIALS SCIENCE, MULTIDISCIPLINARY                                  & 20                  & 23                 \\ \hline
\end{tabular}


==> CAS Journal Ranking/table/top_20_fncsi_fnif.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Journal}     & \textbf{FNCSI} & \textbf{journal}     & \textbf{FNIF} \\ \hline
LANCET               & 1                       & CA-CANCER J CLIN     & 1                      \\ \hline
NATURE               & 2                       & NEW ENGL J MED       & 2                      \\ \hline
JAMA-J AM MED ASSOC  & 3                       & LANCET               & 3                      \\ \hline
SCIENCE              & 4                       & JAMA-J AM MED ASSOC  & 4                      \\ \hline
CELL                 & 5                       & NATURE               & 5                      \\ \hline
WORLD PSYCHIATRY     & 6                       & PSYCHOL SCI PUBL INT & 6                      \\ \hline
LANCET NEUROL        & 7                       & Q J ECON             & 7                      \\ \hline
NAT PHOTONICS        & 8                       & WORLD PSYCHIATRY     & 8                      \\ \hline
NAT GENET            & 9                       & SCIENCE              & 9                      \\ \hline
NAT MED              & 10                      & LANCET ONCOL         & 10                     \\ \hline
NAT MATER            & 11                      & LANCET NEUROL        & 11                     \\ \hline
LANCET ONCOL         & 12                      & NAT MATER            & 12                     \\ \hline
CANCER CELL          & 13                      & NAT GENET            & 13                     \\ \hline
NAT CHEM             & 14                      & PSYCHOL BULL         & 14                     \\ \hline
NAT NEUROSCI         & 15                      & CELL                 & 15                     \\ \hline
CELL METAB           & 16                      & NAT ENERGY           & 16                     \\ \hline
LANCET RESP MED      & 17                      & NAT PHOTONICS        & 17                     \\ \hline
NAT IMMUNOL          & 18                      & CIRCULATION          & 18                     \\ \hline
LANCET DIABETES ENDO & 19                      & FUNGAL DIVERS        & 19                     \\ \hline
NAT NANOTECHNOL      & 20                      & LANCET INFECT DIS    & 20                     \\ \hline
\end{tabular}

==> CAS Journal Ranking/table/top_prob.tex <==
\begin{tabular}{|c|c|c|c|}
\hline
\rowcolor[HTML]{C0C0C0} 
\textbf{Journal} & \textbf{Rank-FNCSI} & \textbf{Rank-Expected   JIF} & \textbf{Rank-JIF} \\ \hline
ECONOMETRICA         & 1  & 69  & 2  \\ \hline
J R STAT SOC B       & 2  & 45  & 3  \\ \hline
ANN STAT             & 3  & 63  & 7  \\ \hline
PROBAB THEORY REL    & 4  & 86  & 10 \\ \hline
ANN PROBAB           & 5  & 103 & 15 \\ \hline
FINANC STOCH         & 6  & 99  & 22 \\ \hline
J AM STAT ASSOC      & 7  & 32  & 4  \\ \hline
INT STAT REV         & 8  & 39  & 16 \\ \hline
J QUAL TECHNOL       & 9  & 104 & 29 \\ \hline
J STAT SOFTW         & 10 & 20  & 1  \\ \hline
ANN APPL PROBAB      & 11 & 60  & 28 \\ \hline
STOCH ENV RES RISK A & 12 & 7   & 8  \\ \hline
BRIT J MATH STAT PSY & 13 & 9   & 20 \\ \hline
TECHNOMETRICS        & 14 & 56  & 21 \\ \hline
BIOMETRIKA           & 15 & 49  & 33 \\ \hline
BAYESIAN ANAL        & 16 & 44  & 35 \\ \hline
BERNOULLI            & 17 & 92  & 41 \\ \hline
INSUR MATH ECON      & 18 & 65  & 43 \\ \hline
EXTREMES             & 19 & 58  & 25 \\ \hline
ECONOMET THEOR       & 20 & 91  & 52 \\ \hline
\end{tabular}
